Does Robustness on ImageNet Transfer to Downstream Tasks?

As clean ImageNet accuracy nears its ceiling, the research community is increasingly more concerned about robust accuracy under distributional shifts. While a variety of methods have been proposed to robustify neural networks, these techniques often target models trained on ImageNet classification. At the same time, it is a common practice to use ImageNet pretrained backbones for downstream tasks such as object detection, semantic segmentation, and image classification from different domains. This raises a question: Can these robust image classifiers transfer robustness to downstream tasks? For object detection and semantic segmentation, we find that a vanilla Swin Transformer, a variant of Vision Transformer tailored for dense prediction tasks, transfers robustness better than Convolutional Neural Networks that are trained to be robust to the corrupted version of ImageNet. For CIFAR10 classification, we find that models that are robustified for ImageNet do not retain robustness when fully fine-tuned. These findings suggest that current robustification techniques tend to emphasize ImageNet evaluations. Moreover, network architecture is a strong source of robustness when we consider transfer learning.

==> fig/fullnetwork_comparison_workshop.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{fig/img/full_network_comparison.pdf}

\end{center}
\caption{
Robust models vs. mean performance drop under 15 corruption types in full-network fine-tuning. 
The lower the performance drop, the more robust models are to these image corruptions.
Regular is a vanilla ResNet50.
DeepAug+ and ANT refer to ResNet50 models robustified via DeepAug+AugMix and ANT, which are all data augmentation techniques to increase robustness against common corruptions \cite{hendrycksManyFacesRobustness2021, rusakSimpleWayMake2020}.
Swin-T is a vanilla Tiny Swin Transformer, where the parameter counts are similar to ResNet50.
If robustness on ImageNet is transferable to other downstream tasks, we would see a similar pattern of ImageNet-C in object detection and semantic segmentation as well. 
However, we see that Swin-T performs much better than DeepAug+, the most robust model against ImageNet-C.
This shows that the Swin Transformer as architecture is a stronger source of robustness transfer than robustification techniques that are used (e.g. DeepAug, AugMix, or ANT).
Moreover, for CIFAR-10, Regular appears to be the most robust model, highlighting the difficulty of transferring ImageNet robustness effectively.}
\label{fig:fullnet_compari}
\end{figure*}
